VFCFinder: Seamlessly Pairing Security Advisories and Patches

Security advisories are the primary channel of communication for discovered vulnerabilities in open-source software, but they often lack crucial information. Specifically, 63% of vulnerability database reports are missing their patch links, also referred to as vulnerability fixing commits (VFCs). This paper introduces VFCFinder, a tool that generates the top-five ranked set of VFCs for a given security advisory using Natural Language Programming Language (NL-PL) models. VFCFinder yields a 96.6% recall for finding the correct VFC within the Top-5 commits, and an 80.0% recall for the Top-1 ranked commit. VFCFinder generalizes to nine different programming languages and outperforms state-of-the-art approaches by 36 percentage points in terms of Top-1 recall. As a practical contribution, we used VFCFinder to backfill over 300 missing VFCs in the GitHub Security Advisory (GHSA) database. All of the VFCs were accepted and merged into the GHSA database. In addition to demonstrating a practical pairing of security advisories to VFCs, our general open-source implementation will allow vulnerability database maintainers to drastically improve data quality, supporting efforts to secure the software supply chain.

==> discussion.tex <==
\section{Discussion - Rename to Threats To Validitiy}
\label{sec:discussion}
\paragraph{Other uses of VFCFinder:}
VFCFinder is a valuable primitive for providing greater transparency for vulnerability fixes and, consequently, will lead to improving the vulnerability database.
It can also be used for more than missing vulnerability-fixing commits for advisories. 
Finding a VFC can lead back to the vulnerability contributing commit~\todocite{VCC} or finding silent fixes~\todocite{cite}. 


\paragraph{Threats to Validity}
As in any research, we have threats to the validity of our evaluation and results.
There is potential for noisy labels within our ground truth data. 
While we randomly sampled our non-VFC commits to confirm the absence of VFCs from within the set, some could be within the remainder set.
The same applies to the VFC data.
We trust the current vulnerability database (NVD, OSV, and GHSA) to provide valid data.
That includes placing trust in the original stakeholder of the reports who filed them with details surrounding the vulnerability patch, such as correct vulnerability fixing commit links. 
We note that prior research has reported errors in NVD data~\todocite{cite}.
Finally, VFCFinder is not able to detect the VFC Type for labels it has not seen. 
For example, we had no examples of ``Vulnerable and Outdated Components" in our training data.
Therefore, when encountering such cases, VFCFinder will likely classify them as \emph{Other}.



==> overview.tex <==
\section{Overview}
\label{sec:overview}

\begin{figure*}[t]
  \centering
  \includegraphics[width=7in]{figures/Overview_Figure_VFC}
  \caption{A high-level architecture of VFCFinder.
  }
  \label{figures:Overview_Figure_VFC}
\end{figure*}


% VFC links in security advisories offer critical information for both practitioners and academic researchers.
% Regrettably, the majority of security advisories, even for open-source projects, lack VFC links.
This paper aims to automate, to the extent possible, the identification of the corresponding VFC from a security advisory for an open-source project.
Realizing this goal necessitates addressing the following research challenges.
  
% \begin{itemize}
%   \item \textit{The open source software ecosystem uses many programming languages.}
%   Previous ML-based tools support a limited number of programming languages (e.g., C/C++, Java, and PHP) owing to the scarcity of labeled training data.

%   \item \textit{Realistic Data Sampling.}
%   Prior work \cite{tan_locating_2021,wang2022vcmatch} uses random sampling techniques for negative samples, drawing 5,000 commits from arbitrary points across a project's version history. Such a method is prone to introducing noise and may also compromise the model's capability in accurately identifying "real-world" patch links. 
%   % We identify that patch links can be expected between the patched and prior version, and the negative samples should be the commits unreleated to the given security advisory.

%   \item \textit{Multiple fixes can occur between version releases.} 
%   Despite potential improvements in VFC identification, existing classification methods are Boolean, limiting the correlation of VFCs with advisories that require understanding the type of fixed vulnerability.

%   \item \textit{Complex approaches.} 
%   Previous research by Wang et al. (2022) \cite{wang2022vcmatch} employs an ensemble of three models and incorporates a high-dimensional feature space with 100 attributes. This extensive feature set raises concerns about the potential for overfitting to the training dataset. 

%   \item \textit{Mapping security advisories to VFCs is manual and time intensive.}
%   Current state-of-the-art tools achieve 88\% accuracy in identifying the VFC within the Top-5 commits~\cite{wang2022vcmatch} and does not apply to the rest of the software supply chain.
%   Sabetta et al. \cite{sabetta_practical_2018} performed a time study and demonstrated that assiting end-users with potential VFCs indeed improve the time for finding the patch link. 
% \end{itemize} 


VFCFinder operates based on the assumption that an advisory's VFC will be situated between the fixed and prior versions (refer to Section~\ref{sec:background}).
Broadly, VFCFinder deems all commits within this window as potential VFCs, and then uses machine learning to provide a ranked list based on the classification confidence.
We opt to segment the overarching classification problem into smaller, distinct classification issues.
This strategy offers several benefits: it renders the classification pipeline more intuitive, enabling domain expertise to guide the classification rather than indiscriminately supplying numerous features to a single ML model; and it allows for the replacement of individual models as research advances.
Finally, VFCFinder combines the individual classification scores using a ranking model, specifically XGBoost~\cite{chen2016xgboost}.
The overall pipeline is depicted in Figure~\ref{figures:Overview_Figure_VFC}.

VFC identification computes the likelihood of a given commit being a VFC, forming a key component of our overall objective.
Earlier work has explored VFC identification through machine learning, examining features such as patch text, commit message text, and associated issue tracker text~\cite{sabetta_practical_2018,giang_hermes_2022,nguyen2022vulcurator}.
However, the state-of-the-art in ML-based VFC identification, VulCurator~\cite{nguyen2022vulcurator}, only achieves an F1 score of 79\%.
During the advisory-to-VFC mapping classification, errors in VFC identification can significantly impact manual confirmation.

VFCFinder relies on prior work to use CodeBERT for VFC identification \cite{nguyen2022vulcurator, nguyen2023multi}.
CodeBERT~\cite{feng_codebert_2020}, an advanced NL-PL transformer-based model by Microsoft, is designed to improve code search and forms the foundation of Microsoft CoPilot~\cite{copilot}.
However, VFC identification differs from code search, thus necessitating fine-tuning CodeBERT with known VFC and non-VFC examples, as described in Section~\ref{sec:vfc_identification}.
Our model trains on a dataset of \totalVFCTrain VFCs from NVD~\cite{nvd}, OSV~\cite{osv_ref}, and VulasDB~\cite{ponta_manually-curated_2019}.
In contrast to the approach outlined in Vulcurator \cite{nguyen2022vulcurator}, our method exhibits comparable performance and superior generalizability, even in the absence of issue linking.
Similiar to Midas \cite{nguyen2023multi}, we also use a fine-granularity prediction scheme, but incorporate the commit message as well. 

VFCFinder also uses CodeBERT for VFC type classification.
Given that a software package's commit window may contain multiple security advisories or even silent vulnerability fixes~\cite{dunlap_2023}, it is vital to identify not just which commits are VFCs, but also their types.
Unlike prior VFC identification techniques, our method classifies the VFC vulnerability type, while DAA~\cite{dunlap_2023}, a non-ML VFC identification approach, can produce a corresponding CWE but has limited recall due to SAST tool reliance.
Parallel to our work, Pan et al. \cite{pan2023fine} classifies the CWE type using CodeBERT and Bi-LSTM models. 
Our work is fine-tuned to classify the OWASP Top-10 and uses only CodeBERT.

Lastly, we augment our advisory-to-VFC mapping classification with three additional features: commit-to-advisory semantic similarity, presence of the CVE or GHSA identifier in commit messages, and the commit rank location.
As detailed in Section~\ref{sec:semantic_similarity}, VFCFinder employs state-of-the-art NLP semantic similarity techniques to compare the commit message with advisory details.
We refer to the last two as "static features," easily extracted from the commit and are intuitive: a commit message featuring the CVE or GHSA identifier should undoubtedly influence the model, and commits closer to the fixed version are more likely to be the VFC.

==> tables/ranking_commits_eval.tex <==
\begin{table}[t]
    % This data comes from ghsa-vfc/wb_vfc_commit_codebert_holdout.py
    % See bottom of file
          % Saves data to ./data/language_generalized_vfc_20221122.csv
    % Need to only look at commits with a single language type
\centering
\caption{Top-N Accuracy for Ranking Commits displayed at the number of commits between the prior and fixed versions of an advisory. For example, 50\% of the GHSA dataset contained less than 15 commits between the prior and fixed versions.}
\label{tbl:ranking_commits_eval} 
\small
\begin{tabular}{lcccc} \toprule
    \textbf{Commit Count} & \textbf{Acc@1} & \textbf{Acc@2} & \textbf{Acc@3} & \textbf{Acc@5} \\ \midrule
    $\leq$ 5 commits (25\% of data)                    & 95.9\%         & 98.8\%         & 99.8\%          & 100\%          \\
    $\leq$ 15 commits (50\% of data)                   & 90.9\%         & 96.1\%         & 98.3\%         & 99.8\%         \\
    $\leq$ 44 commits (75\% of data)                   & 85.8\%         & 93.9\%         & 96.9\%         & 99.0\%         \\ \midrule
    Total Test Dataset                          & 80.0\%         & 89.5\%         & 93.2\%         & 96.6\%         \\ \bottomrule
\end{tabular}
\normalsize
\end{table}

% The number of commits only impact a single project (the number of commit is static between a project). The classification is between the window of an advisory.

==> tables/vfc_baseline.tex <==
\begin{table}[t]
      % This data comes from CWEClassification/wb_vfc_commit_codebert_hermes.py
      % 10-fold see EPOCH 5 from the first fold
      % In future try to run the pre-trained VFCFinder on the same data maybe
\centering
\caption{VFCFinder baseline comparison against Sabetta et al.~\cite{sabetta_practical_2018}, HERMES~\cite{giang_hermes_2022}, and VulCurator~\cite{nguyen2022vulcurator} on their Java Dataset for VFC Identification.}
\label{tbl:vfc_baseline}
% \begin{tabular}{llll} \toprule
% Model                                        & Precision & Recall & F1   \\ \midrule
% Sabetta et al.~\cite{sabetta_practical_2018} & 0.54      & 0.82   & 0.64 \\
% HERMES~\cite{giang_hermes_2022}              & 0.80      & 0.67   & 0.72 \\
% VulCurator~\cite{nguyen2022vulcurator}       & 0.80      & 0.67   & 0.72 \\
% VFCFinder                                    & 0.91      & 0.83   & 0.87 \\ \bottomrule
% \end{tabular}
\small
\begin{tabular}{lll} \toprule
      \multicolumn{1}{c}{\textbf{Model}}                & \multicolumn{1}{c}{\textbf{Approach}} & \multicolumn{1}{c}{\textbf{F1}}   \\ \midrule
      Sabetta et al.~\cite{sabetta_practical_2018}      & Message + Code (BoW)  & 0.64$^*$ \\
      HERMES~\cite{giang_hermes_2022}                   & Message + Issue + Code (SVM)   & 0.68$^\dagger$ \\
      VulCurator~\cite{nguyen2022vulcurator}           & Message + Issue + Code (CodeBERT) & 0.79$^\dagger$ \\
      VFCFinder                                          & Message + Code (CodeBERT)   & 0.87 \\ \bottomrule
      \multicolumn{3}{l}{\footnotesize $^*$ As reported by HERMES~\cite{giang_hermes_2022}; $^\dagger$ As reported by VulCurator~\cite{nguyen2022vulcurator}.}
      \end{tabular}
\normalsize
\end{table}

==> vcmatch.tex <==
\section{VCMatch}
\label{sec:vcmatch}

We compare against VCMatch directly.
VCMatch uses 100 features that from the patch link and security advisory. 
VCMatch only targets three languages (C/C++, PHP, and Java) unlike our comparison of nine different languages.

The sampling approach for training and testing in both PatchScout and VCMatch suffer from data leakage, thus inflating their results.
Also, the 10 open source projects they evaluated against have some of the best documented commits among open source projects.
For example, the vulnerability fixing commits are highly descriptive and can trivially be matched back to the advisory. 

We directly compare against VCMath in two ways.
1. We run VFCFinder directly on their dataset to demonstrate their data is over-simplified compared to other datsets.
2. We run VCMatch on our testing set to demonstrate that VCMatch does not generalize to other languages and realworld data.
The trained models of VCMatch were released in their recent work PatchMatch (a GUI based implementation of VCMatch).

\paragraph{title}
